Twins: BFT Systems Made Robust

This paper presents Twins, an automated unit test generator of Byzantine attacks. Twins implements three types of Byzantine behaviors: (i) leader equivocation, (ii) double voting, and (iii) losing internal state such as forgetting 'locks' guarding voted values. To emulate interesting attacks by a Byzantine node, it instantiates twin copies of the node instead of one, giving both twins the same identities and network credentials. To the rest of the system, the twins appear indistinguishable from a single node behaving in a 'questionable' manner. Twins can systematically generate Byzantine attack scenarios at scale, execute them in a controlled manner, and examine their behavior. Twins scenarios iterate over protocol rounds and vary the communication patterns among nodes. Twins runs in a production setting within DiemBFT where it can execute 44M Twins-generated scenarios daily. Whereas the system at hand did not manifest errors, subtle safety bugs that were deliberately injected for the purpose of validating the implementation of Twins itself were exposed within minutes. Twins can prevent developers from regressing correctness when updating the codebase, introducing new features, or performing routine maintenance tasks. Twins only requires a thin wrapper over DiemBFT, we thus envision other systems using it. Building on this idea, one new attack and several known attacks against other BFT protocols were materialized as Twins scenarios. In all cases, the target protocols break within fewer than a dozen protocol rounds, hence it is realistic for the Twins approach to expose the problems.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#

TEX = paper
FIGS = 
PSFIGS = $(FIGS:.pdf=.ps)

all: pdf
ps:  $(TEX).ps
pdf: $(TEX).pdf
dvi: $(TEX).dvi

clean:
	$(RM) *.synctex.gz *.out *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx *.eps dummy
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

# only need -Ppdf if using CM fonts

paper.pdf: *.tex *.bib Makefile
	pdflatex paper.tex
	bibtex paper
	pdflatex paper.tex
	pdflatex paper.tex


==> sections/conclusion.tex <==
\section{Conclusion}

\label{conclusion}

Conclusion.

==> sections/fab.tex <==
% ==========
% FAB
% ==========
\section{Expressing Attacks on \fab as Twins}
\label{sec:fab}
We present a summary of \fab~\cite{fab}, and express an attack against its liveness introduced by Abraham~\etal~\cite{abraham2018revisiting} in the context of \Twins. 

% ==========
\subsection{Summary of \fab} 

\label{sec:fab-summary}


% ==========
\subsection{Attacks on \fab} \label{sec:fab-attacks}
We demonstrate that a progress-certificate may contain $f + t + 1$ new-view messages with some prepare value, and a commit-certificate with a different value. This causes $\fab$ to get stuck because there is no value vouched-for by the certificate, hence new leaders cannot make any valid proposal. For a scenario, we set $f = 1, t = 0, n = 3f + 2t + 1 = 4$. Denote the replicas by A, B, C, D, where D has a twin D'. The scheduler produces the following schedule:
\begin{description}
\item [Step 1] Initialize D and D’ with different inputs d and d’. 

\item [Step 2] During View 1:
\begin{itemize}
\item Run D as leader for one round. 
\item When D proposes d, allow the proposal from D to be delivered only to A and B. 
\item D, A, and B accept the proposal and send \textit{prepare} messages; but the scheduler allows these messages only to reach A. Thus, only A produces a \textit{commit-certificate} for the value d.
\item Meanwhile, the leader D' equivocates and pre-proposes d' to C.
\end{itemize}

\item [Step 3] Delay all further messages until new view starts; set A as leader of this new view. The new leader A collects a \textit{progress certificate} consisting of new-view messages (REP) from a quorum of 3 replicas (including itself):
\begin{itemize}
\item from D', the new-view message contains the value d', and no commit-certificate.
\item from A, the new-view message contains the value d, and a commit-certificate for it.
\item from C, the new-view message contains the value d', and no commit-certificate.
\end{itemize}
\end{description}
Now we are stuck. This progress certificate contains 2 messages (from D' and C) with prepare value d'. Hence, the certificate does not vouch for d. At the same time, it contains a commit-certificate (from A) with value d; hence, it does not vouch for d' either. As mentioned by Abraham~\etal~\cite{abraham2018revisiting}, The \fab paper includes an argument that all process certificates vouch for at least one value (Lemma 7), but unfortunately it has a mistake.


==> sections/knownattacks-old.tex <==
\section{Known Attacks}

\label{known-attacks}
\alberto{Use different macros for twins approach and twins implementation (make them self-contained). Move this section before section 5?}

In this section, we proceed to show 
that several famous attacks on \bft consensus protocols
are reinstated by the \Twins approach.
In all cases, exposing flaws requires only one or two leader rotations and
small number of nodes.
We will show in Section~\ref{generator} that running an automated scenario generator with these configurations would cover these scenarios within minutes.
We did not undertake to fully implement these
protocols, but rather, they are demonstrated using the notation introduced in
Section~\ref{notation}.

The following attacks are re-instated in \Twins:

\begin{description}

\item[\zyzzyva]
\zyzzyva broke new ground in BFT replication with the introduction of
an optimistic single phase ``fast track''.
Eleven years elapsed from its publication until a safety flaw in \zyzzyva was discovered~\cite{abraham2018revisiting},
during which numerous research project and systems were built over it. As
demonstrated below, \Twins generates a scenario that exposes the flaw with 4
nodes and two leader rotations: the first leader equivocates via a twin, the next two leaders drop messages to/from some nodes. \alberto{The following sentence is not clear.} This scenario is among $30K$ ones that the \librabft \Twins scenario generator enumerates and tests in under 1 minutes. \todo{Alberto: please
check the numbers} 

\item[\fab]
A precursor to \zyzzyva, \fab~\cite{fab} is a view-based protocol with an optimistic fast
track. Not surprisingly, a similar problems arises in \fab due to a flawed leader replacement protocol~\cite{abraham2018revisiting}, albeit manifesting as a liveness bug. \Twins exposes this bug in under one minute, in a short scenario with $n=4$ and three leader rotations, leading to a complete absence of leader proposals.

\item[\synchs]
``Force-Locking Attack''~\cite{momose2020force} is a timing attack on a preliminary version of a synchronous BFT protocol named \synchs~\cite{synchs} (which was subsequently updated to resist the attack). As before, this attack requires only a small system size, $n=5$, and two leader rotations. However, in order to create timing attacks, scenarios need to include timing information for protocol steps and messages deliveries. Extending our scenario generation strategy with timing data is left for future work. In the specific attack at hand, course-grain timing at fixed intervals---fewer than ten---suffice to reinstate the attack.

\item[\tendermint]
\tendermint~\cite{tendermint} is a view-based protocol that builds on the classical two-phase PBFT~\cite{pbft} algorithm, but greatly simplifies the leader replacement protocol. However, even when communication is timely, progress may be prevented indefinitely~\cite{latest-gossip-in-tendermint,hotstuff-paper}. Detecting the lack of progress can be done by observing that two consecutive views with honest leaders whose communication with a quorum is timely do not produce a decision.   

\end{description}
% --------------------

\todo{Dahlia: I believe all the detailed scenarios below could go to an appendix if needed.}
% ------- Zyzzyva ----------

\subsection{\zyzzyva} 
\label{sec:zyzzyva}

% --------------------

\para{Summary of \zyzzyva}
%
\zyzzyva is an SMR protocol in the same settings as \librabft (partial synchrony
and $n=3f+1$). It operates in a view-by-view manner. Each view has a designated leader. 
Nodes vote on the leader proposal if they consider it valid (we describe the validity criteria below, which has a flaw that enables the safety attack).
A commit decision on the leader proposal forms in either of two tracks,
fast and two-phase. In the fast track, all $n$ nodes vote for the leader
proposal to commit it. In the two-phase track, $2f+1$ nodes form a
commit-certificate (\cc), then $2f+1$ nodes vote for the \cc to commit
the proposal.


At the beginning of the view, nodes send the
new leader a signed NEW{-}VIEW status message. 
The leader's first proposal carries the status of $2f+1$ nodes at the beginning
of the view to prove the proposal validity.
The (flawed) definition in \zyzzyva for a valid proposal upon view change is as
follows. For each sequence slot:
\begin{itemize}
    \item \textbf{Validity Rule 1} The leader picks among the states of $2f+1$ nodes, the \cc from the highest view, if one exists.
    \item \textbf{Validity Rule 2} Otherwise, the leader picks a proposal that has $f+1$ votes from the highest view, if one exists.
    \item \textbf{Validity Rule 3} Finally, if none of the above exist, the leader creates a Nil proposal.
\end{itemize}

The flaw is to prioritize Validity Rule 1 over Validity Rule 2, which causes the leader to prefer \cc even if generated in a \emph{lower view} than $f+1$ votes.

% --------------------

\para{Safety Attack on \zyzzyva} 
%
\label{sec:zyzzyva-attacks}
%
The \zyzzyva flawed scenario safety demonstrated in~\cite{abraham2018revisiting} goes through a succession of three views. 
%
In the first view, a faulty leader generates conflicting proposals $V_1, V_2$ and splits honest nodes between $f+1$ that vote for $V_1$ and $f$ that vote for $V_2$. The faulty leader gathers a \cc on $V_1$ but does not send it to other nodes. 
%
In the second view, a good leader adopts $V_2$ and drives agreement in the fast track. 
%
In the third view, $f$ faulty nodes join the $f+1$ honest nodes that voted for $V_1$ in the first view. They send the leader a \cc for $V_1$,
hence the protocol proceeds with $V_1$, in conflict with the $V_2$ commit.
%
The attack on \zyzzyva needs only $n=4$ nodes, of which $f=1$ is faulty, and it is fairly easy to re-instate using the \Twins framework. There are four nodes, $(D, E, F, G)$. To model the case that $D$ is \Byzantine, it has a \twin $D^\prime$ initialized with different input.
We drive the execution creating partitions and electing leaders at each step, according to the attack described above.
% \bano{Commenting the below. It doesn't provide enough information to understand the attack. Interested readers will go to the appendix.}
% The network scheduler partitions the nodes in the first view to $\{D, E, F\}, \{D', G\}$. 
% In the second view, it isolates $\{D\}$ and delivers NEW{-}VIEW messages to $G$ first from $\{D^\prime, E\}$. 
% In the third view, it partitions to $\{D, E, F\} \{D^\prime, G\}$.
We describe the detailed attack using \Twins in Appendix~\ref{zyzzyva-detail}.

% --------------------

% -------- FAB --------

\subsection{\fab}
\label{sec:fab}

\todo{Dahlia: because Fab and Zyzzyva are similar, we can move all the text on FaB below here to the appendix, if we need the space.}

% --------------------

\para{Summary of \fab} 
%
\fab is a single-shot consensus protocol for the partial synchrony setting with
$n=3f+1$.\footnote{FaB is actually designed for a \emph{parameterized} model with
$n=3f+2t+1$, with safety guaranteed against $f$ Byzantine failures and fast track
guaranteed against $t$. For brevity and uniformity, we ignore $t$ here and set
$t=0$.}

A precursor to \zyzzyva, \fab is a view-based protocol with an optimistic fast
track. A leader drives a decision in the fast track if all nodes vote for it,
and in the two-phase track if $2f+1$ nodes vote for a $(2f+1)$
commit-certificate (\cc). When a new leader is elected, it picks a valid proposal that does not conflict with neither $f+1$ votes nor a \cc in the previous view.

% --------------------

\para{Liveness Attack on \fab} \label{sec:fab-attacks}
%
The (flawed) selection criterion above leads an execution in the following scenario to become stuck. A faulty leader equivocates and proposes $V_1, V_2$ to $2f+1$ and
$f$ honest nodes, respectively. In transitioning to the next view, there is
a commit-certificate for $V_1$ and $f+1$ votes 
for $V_1$ (including an equivocation by one faulty), hence neither is safe,
and the new leader is stuck.
The attack on \fab needs only $n=4$ nodes, of which $f=1$ is faulty, and it can be easily re-instated using \Twins. There are four nodes, $(A, B, C, D)$ with $D$ as a \Byzantine node, for which we create a \twin $D^\prime$ initialized with different input.
We describe the attack using \Twins in detail in the Appendix~\ref{fab-detail}.

% --------------------

% -------  HotStuff Synch -----------

\subsection{Timing Attack on \synchs}
\label{sec:synchs}


\para{\synchs in a Nutshell} 
%
The preliminary version of~\synchs~\cite{synchs} is an \smr solution in the synchronous model with $n=2f+1$ parties.\footnote{The description here covers the first of three 
variants in that paper; two other variants 
are designed for slightly different synchrony assumptions, but the attacks
on them are similarly covered by the \Twins approach.} 

In synchronous protocols like \synchs, nodes execute the protocol in terms of $\Delta$, which is the known bound assumed on maximal network transmission delay.
\synchs operates in a view-by-view regime 
%which is the hallmark of partial-synchrony solutions.
---in each view there is a designated leader which proposes values to nodes.
If a node accepts the proposed value, it broadcasts its vote.
A node creates a commit certificate (\cc) for a proposed value if it receives $f+1$ votes on it.
Nodes track the highest \cc, and only vote on a proposed value if it: \first extends the highest \cc known to the node, and \second does not equivocate another value proposed for the same height.

A node creates and broadcasts a \emph{blame} against a leader: \first if the leader does not propose a value for $3\Delta$, or \second the leader proposes an equivocating value. 
If a node observes $f+1$ blames against the leader in the current view, it broadcasts the $f+1$ blames, then waits $\Delta$ (to allow the blames to reach all honest nodes), and moves to the new view. 
In the new view, it immediately sends the new leader
the highest \cc it knows of.

After a view change, the new leader waits 
%2\Delta$ 
for $\Delta$ to receive node status messages (carrying the highest \cc known to them).
The leader then proposes a value that extends the highest \cc from among the received status messages.
Nodes proceed in the new view as previously described.
%to start and sends a proposal carrying the highest view it knows. 
% Nodes broadcast a vote for the proposal if it does not conflict with any other proposal carrying a
% certificate of the same view or higher. A commit decision on the leader proposal is
% reached if no conflicting proposal is received within $2\Delta$. 
% If there is no progress for $3\Delta$, a node blames the leader to affect a view
% change.

% --------------------

\para{Implementing Synchrony Attacks in \Twins} 
%
Due to the synchronous settings and the nature of the attack which heavily
leverages synchrony assumptions, in this case a \Twins scheduler must control message delivery timing. 
More precisely, rather than only specifying whether a message is delivered to a party or dropped, attacks on synchronous protocols require the \Twins scheduler to deliver messages to specific parties at specified times.
While this is captured by the \Twins approach, our current implementation  (Section~\ref{implementation}) does not support this feature (this will be implemented in future \Twins extensions).

Generally, we expect that the granularity of the scheduler timing can be fairly coarse. In particular, there is a known
parameter $\Delta$, the bound presumed by the algorithm on message transmission delays and hard-coded into it. 
Indeed, the \forcelocking attack needs to deliver messages at $0.5 \Delta$ increments, \eg at times $0, 0.5\Delta, \Delta, 1.5\Delta,
2.0\Delta, ..$. Therefore, a \Twins network emulator could operate in discrete lock-step at $0.5\Delta$ increments.
With this capability in place, the \forcelocking attack can be re-instated in the \Twins approach as described below. 

% --------------------

\para{Safety Attack on \synchs} \label{sec:synchs-attacks}
%
We now rebuild the \forcelocking attack on the preliminary version of \synchs using \Twins.
% described
% above which is inspired by the Momose attack\footnote{The original
% attack assumes faulty parties would deliberately ignore timing violations. We
% cannot make this assumption with \Twins, but can modify the attack to work
% without such constraint.} 
The crux of the attack is for a faulty leader to generate a last-minute
proposal that reaches only half of the honest nodes. 
The other half trigger a view change, and now the system becomes split. 
The first half continues to commit the first leader proposal with ``help'' from \byzantine nodes. The second half starts a new view and fork the chain.
This attack can be reinstated with \Twins using 5 nodes $(A, B, C, D, E)$, of which $(A, B)$ are faulty and have \twins $(A^\prime, B^\prime)$. 
The detailed attack using \Twins appears in Appendix~\ref{synchs-detail}.

% To reinstate this attack with \Twins, we deploy seven replicas $B, C, D, E, F,
% G, H$, of which $C, D, E$ are faulty and have \twins $C', D', E'$ . 
% The scheduler relays the first leader $D$ proposal through $F$ and on to $G$
% incurring the maximal $\Delta$ delay at each hop.
% $G, H$ receive the proposal before expiring the first view. $B, C$ will
% eventually receive it through $G, H$ only after they accuse the leader. 

% To emulate bad behavior by $F$, the \twin $F'$ will receive the
% leader message only after the expiration, like $G, H$. Jointly
% $B, C, E, F'$ form a quorum that initiates a new view and proceed to fork $D$'s
% proposal. Meanwhile, $G, H$ collects a certificate on $D$'s proposal that
% prevents the fork from surviving.
% The detailed scenario appears in the appendix.

% --------------------

\subsection{Liveness Attack on \tendermint}

\label{sec:tm}

\para{\tendermint in a Nutshell}

A precursor to \hotstuff~\cite{hotstuff} and to \librabft~\cite{librabft},
\tendermint operates in two-phase views, but suffers from a liveness problem
that \hotstuff/\librabft solve by adding a third phase. 

\tendermint operates in a view-by-view manner. Each view has a designated leader
collecting transactions into a block and proposing a block that extends the
highest \qc it knows. 
Nodes vote on the leader proposal if they consider it extends the highest \qc
they know.
A commit decision on the leader proposal forms if $2f+1$ nodes form a
quorum-certificate (\cc) and then $2f+1$ nodes vote for the \qc to commit
the proposal.

Progress is hinged on leaders obtaining the highest \qc from the system through
gossip. Therefore, liveness is broken if leaders are repeatedly excluded from 
the gossip of \qc's. 

More specifically, the liveness attack on \tendermint uses 4 replicas $(D,E,F,G)$, where $D$ has a twin $D^\prime$.
In the first view, $D$ and $D^\prime$ generate equivocating proposals. 
Only $D, E$ receive a \qc for $D$'s proposal. 
The next leader is $F$ who proposes to 
% \bano{There is no \cc on this proposal, so it can be re-proposed but not extended}
%extend 
re-propose
the proposal by $D^\prime$, which $E$ and $D$ do not vote for because they already have a \cc for that height. 
Only $F$ and $D^\prime$ receive a \qc for $F$'s proposal. 
This scenario repeats indefinitely, resulting in loss of liveness.
The detailed attack using \Twins appears in Appendix~\ref{tm-detail}.


==> sections/limitations.tex <==
\myparagraph{Limitations \& Scope.}
%
We recognize that (setting aside trivial, easily filtered formatting violations)
some Byzantine behaviors are not covered by \Twins. 

For one, in some protocol
steps, a node may wait for messages to determine its next action. Under \Twins,
the node is forced to act according to the messages it received, as if the node
provided a justification for each step in form of the history of messages it
received. Deviating from this behavior was not required to reinstate any of the attacks discussed in \Cref{known-attacks}, though in principle, various deviating behaviors would not be covered by \Twins. 
%
Another coverage challenge emerges in synchronous protocols because a node behavior may be based on real time. In such protocols, \Twins essentially forces a node to behave in a timely manner. We tackle this case in one of the attacks investigated in Section~\ref{known-attacks} and demonstrate that nonetheless, a slight adaptation of the original attack reinstates the attack in \Twins. However, we do not know yet which timing attacks may not be covered.  

Additional challenges stem from pragmatic needs. In particular, 
while the \Twins approach allows creating up to $k$ instances of a node, throughout this paper we set $k=2$. The \byzantine behavior emulated by \Twins involves equivocation or duplication, which needs only two messages to diverge or match.
This choice helps us cover interesting cases, while pruning potentially redundant \testcases due to higher values of $k$.
It is unknown yet which safety violations can only be covered by $k>2$.
 

Finally, this paper explores the use of \Twins to expose safety and liveness violations---the principal properties of \bft systems. There are other properties of \bft systems such as transaction inclusion and fairness~\cite{fair-ordering,censorship}
%\bano{Find a way to rephrase this so we don't use the controversial word, censorship \alberto{What about simply 'decentralization' (even if it is not exactly the same thing)?}}, 
and performance bounds~\cite{prime}, that \Twins can be extended to verify. 
%Similarly, \Twins does not model attacks involving misformed messages, for which existing techniques such as fuzz testing are more suitable.  

Increasing coverage of \Twins in the settings we explore as well as others, and providing a formal treatment of coverage remain 
interesting open challenges; we discuss some concrete future directions in
Section~\ref{future}. 

% DM: removed, do we need this? The introduction is becoming rather long.
%\myparagraph{Roadmap}
%The rest of this paper is structured as follows. 
%
%Section~\ref{scenarios} provides an overview of \Twins, describing how concrete attack scenarios can be modeled by \Twins. 
%
%Section~\ref{design} describes the design of \Twins and discussed how concrete attack scenarios can be modeled by \Twins. 
%
%followed by implementation (Section~\ref{implementation}) and evaluation (Section~\ref{evaluation}). In Section~\ref{known-attacks}, we show how famous attacks on \bft consensus can be reinstated by \Twins. We provide a comparison with related work in \Cref{related}. We discuss future directions and conclude the paper in \Cref{future}. 


% \bano{TODOs: Things to do globally, through the rest of the paper.}
%
% Use US English
% Use Cref consistently.
% Use separate macros for Twins implementation (\TwinsImpl) and Twins approach (\Twins).
% Ensure notation is consistently used (especially using P for partitions and small v for proposed values).
% Use \testcases macro. Prefer \testcase over scenario
% Use the macro \twin for referring to a twin node, \Twins is for the approach.
% The word 'reinstate' is overused. Fix, if possible.
% Use single v/s double quote consistently
% Spell out quorum certificate (or timeout certificate) only the first time in a section, and then use QC (or TC)
% Make biblio complete and consistent

==> sections/semisync.tex <==
\section{\Twins in the Synchronous Model}

Working on synchronous settings surfaced a potentially interesting challenge.

The original attack by Momose required a Byz faulty party to deviate from the
protocol timing. Specifically, the original attack assumes execution starts at
time $t_0$ (for everyone). Then it delays the first Byz leader from sending a
proposal until $t_0 + 2.5\Delta$. 

This behavior might not be possible to emulate with the Twins approach if the code executed by a participant could notice that too much time has elapsed. In that case, the leader itself would recluse itself from proposing.  

However, it seems that for the same reason, it is equally easy for a protocol to defend against such Byz behavior (without fixing the actual logical bug). 

The idea is to force protocols in the synchronous settings to use a
\emph{semi-synchronous transport}. 

\subsection{Semi-Synchronous Transport}

Assume that (in synchronous settings) the start of each protocol step is
synchronized up to $\Delta$ discrepancy. This is a reasonable assumption, because
(ignoring message complexity) each node can broadcast when it starts a new step
and piggyback a justification that causes any party the receives the broadcast
to switch to the new step. For example, in Sync HS, any node can broadcast a
``wake up and start'' message at the beginning and cause everyone to start
within $\Delta$ of one another. Similarly, in Sync HS, whenever a node wants to
move to a new view, it already broadcasts a vector of $f+1$ ``blame'' messages, causing everyone to enter the new view within $\Delta$ of one another. 

To further implement a semi-synchronous transport, a node will drop a message
for step $t_x$ if it arrives more than $2\Delta$ after step $t_x$ has been announced. 

I will try to argue that Twins capture timing attacks under the semi-synchronous
transport execution model.

Indeed, with a semi-synchronous transport, perhaps the most that a bad
node can do in an attack is delay for $2\Delta$ (instead of one $\Delta$). Then
we can argue that \Twins can emulate this by delaying the delivery of ``next
step'' broadcasts to the bad node by $\Delta$, and then another $\Delta$ for the propagation of the message the node sends.

\subsection{Does \Twins Capture all Timing Misbehaviors?}

Wrapping back to the Momose attack, I went back to see whether the timing
violation was crucial.
I managed to re-create the attack under the semi-synchronous transport model. I created a chain of 3 hops from
the leader. I made each hop take $\Delta$ time, and assumed the leader starts at $.5Delta$ due to discrepancy in
local clocks. (BTW, in order to have a chain of two faulty nodes and leave one
more faulty node for the attack, I had to use $f=3$, $n = 2f+1 = 7$ nodes.) 

The original attack is not possible under
the semi-synchronous transport.  The modified attack is possible with a
semi-synchronous transport but Twins captures it. 

This to leads to an interesting question.  Is there a class of timing attacks that Twins cannot capture? 


==> sections/streamlet.tex <==
\section{Attack on Modified Streamlet} 

\label{sec:streamlet}

We inject a bug into Streamlet~\cite{chan2020streamlet} (similar to \Cref{validation}), and use \Twins to instantiate a liveness attack that exploits the injected bug.

\subsection{Summary of Streamlet}
Streamlet is a protocol for the partially synchronous setting with $n=3f+1$ known nodes, up to $f$ of which may be \byzantine. The network has an unknown global stabilization time (GST), after which there is a known duration $\Delta$ (measured in rounds) that bounds all transmission delays between honest nodes.
%
Streamlet is an epoch-by-epoch protocol with a known designated leader per epoch. In each epoch, a leader broadcasts a proposed block carrying transactions. 
%As previously done in HotStuff, 
Each proposed block is chained to a quorum-certificate (QC) of $2f+1$ votes on a previous block (or the genesis block).

Streamlet requires epochs to start in full synchrony and to last $2\Delta$ rounds. Under this assumption, Streamlet guarantees that a block will be finalized after GST whenever a succession of 5 epochs with honest leaders occurs.

\para{Voting and commit rules}
Every node keeps the longest chain \emph{highQC} that it knows; a leader proposal extends \emph{highQC}, and a node votes for a leader proposal if it extends the branch of its \emph{highQC}. Whenever a 3-chain of alternating block-QCs with  consecutive epochs is formed, the middle block of the 3-chain becomes finalized.


\subsection{Liveness Attack on Modified Streamlet} \label{sec:streamlet-attack}
We modify Streamlet as follows: instead of extending the longest chain, each node extends the \emph{highest epoch}.

We then use \Twins to demonstrate that the modified Streamlet does not finalize a new block even after GST and despite 5 consecutive epochs of honest leaders. In fact, progress is not guaranteed even with an indefinite number of consecutive honest leaders.
%
In a nutshell, \Twins generates round-by-round scenarios. In a scenario, each round can partition the honest nodes into two (or more) subsets, such that messages from bad parties arrive only at one subset. Using such scenarios, \Twins generates Streamlet epochs in which votes are collected into a partially-known QC that arrives at only a single honest node. 
%Building epochs with partially-known QCs in succession, the protocol may exhibits no finalized blocks despite any number of repetitions of the main loop.
Due to successive epochs with partially-known QCs, the protocol may never finalize any blocks thus losing liveness.

\para{Before GST}
\begin{itemize}
    \item An epoch-1 block is proposed.
    \item Due to the lack of synchrony, $2f+1$ votes for the epoch-1 block arrive in time $2\Delta$ only to one honest party denoted $V1$.
\end{itemize}

\para{After GST}
\begin{itemize}
    \item Set $V_{prev}$ to $V1$.
    \item Set $B_{prev}$ to the epoch-1 block.
    \item For each epoch $e$: \ \
    \begin{enumerate}
        \item A leader $L \neq V_{prev}$ broadcasts an epoch-e proposal conflicting with $B_{prev}$.
        \item $2f$ honest nodes vote for epoch-$e$, but $V_{prev}$ does not vote for epoch-e because it does not extend $B_{prev}$, the block with the highest QC known to $V_{prev}$.
        \item One bad node sends a vote on epoch-e that reaches only one honest party $V_x$ right at the end of epoch $e$. That is, at the end of epoch $e$, a QC for the epoch-$e$ block (that includes a vote from one bad participant) arrives to only one honest node $V_x$.
        \item Set $V_{prev}$ to $V_x$.
        \item Set $B_{prev}$ to the epoch-$e$ block.
    \end{enumerate}
\end{itemize}

\para{Expressing the attack as \Twins}
There are four nodes, (D, E, F, G). We describe below the detailed attack using \Twins:
\begin{description}
\item [Epoch 0 (before GST)]: \begin{itemize}
    \item Create the following partitions: $P_1 = \{E, G\}, P_2 = \{D, E\}, P_3 = \{E, F\}$. Those partitions allow $E$ to communicate with all nodes, but all other nodes can only communicate with $E$; this is allowed as it happens during a period of asynchrony.
    \item Let $E$ be the leader. $E$ proposes $v_0$, gathers votes from $(D, F, G)$ and creates $QC(v_0)$; its highest QC is $QC(v_0)$.
\end{itemize} 

\item [Epoch 1]: \begin{itemize}
    \item Create the following partitions: $P_1 = \{E, F, G\}, P_2 = \{D, F\}$.
    \item Let $F$ be the leader. $F$ proposes $v_1$, gathers votes from $(F, E, G)$ and creates $QC(v_1)$; its highest QC is $QC(v_1)$. $E$ does not vote on $v_1$ as it does not extend its highest QC $QC(v_0)$, so only $F$ obtains $QC(v_1)$ in this epoch.
\end{itemize} 

\item [Epoch 2]: \begin{itemize}
    \item Create the following partitions: $P_1 = \{E, F, G\}, P_2 = \{D, E\}$.
     \item Let $E$ be the leader. $E$ proposes $v_2$, gathers votes from $(D, E, G)$ and creates $QC(v_2)$.
\end{itemize} 

\item [Epoch 3]: Same as Epoch 1.

\item [Epoch 4]: Same as Epoch 2.

\item [Epoch 5]: Same as Epoch 1.
\end{description}

\subsection{Implementation of the Attack} \label{sec:streamlet-impl}
We implement a simulator of Streamlet in Python, using the discrete event simulator \emph{simpy}\footnote{\url{https://pypi.org/project/simpy/}}.
%rather than a real network. 
The simulator takes as input \Twins scenarios produced by the \Twins generator (see \Cref{generator-impl}) and runs the protocol under the conditions specified by the scenario (\ie number of nodes, number of \twins, number of rounds, partitions per round, and leaders per round). We run the \Twins scenarios against  a modified version of the Streamlet simulator with the bug presented in \Cref{sec:streamlet-attack}, and observe the liveness attack using a manually-crafted scenario. We are open sourcing our Streamlet simulator, both the modified (buggy) and the correct protocol versions\footnote{
\ifdefined\cameraReady
\url{https://github.com/asonnino/twins-simulator}
\else
Link removed for blind review.
\fi
}.

==> sections/tmdetail.tex <==

\section{Detailed Liveness Attack Scenario on Linear View-Replacement} 

\label{tm-detail}

We use \Twins to demonstrate a liveness attack~\cite{abraham2018revisiting} on \tendermint.
A brief summary of \tendermint and the attack described below is provided in~\Cref{sec:tm}.
We denote a commit-certificate, \ie $2f+1$ votes on a value, as \cc. 
The attack uses 4 replicas $(D,E,F,G)$, where $D$ has a twin $D^\prime$.

More specifically, the liveness attack on \tendermint uses 4 replicas $(D,E,F,G)$, where $D$ has a twin $D^\prime$.
In the first view, $D$ and $D^\prime$ generate equivocating proposals. 
Only $D, E$ receive a \qc for $D$'s proposal. 
The next leader is $F$ who proposes to extend the proposal by $D^\prime$, which $E$ and $D$ do not vote for. 
Only $F$ and $D^\prime$ receive a \qc for $F$'s proposal. 
And so on.

%
\begin{description}
% -------- Step 1 ------
\item [Step 1] Initialize $D$ and $D^\prime$ with different inputs $V_1$ and $V_2$. 

% -------- Step 2 ------
\item [Step 2] During View 1:

\begin{itemize}

\item Create the following partitions: $P_1=\{\underline{D},E,G\}$, $P_2=\{\underline{D^\prime},F\}$.

\item Let $D$ and $D^\prime$ run as leaders for one round. $D$ proposes $V_1$ to $P_1$ and gathers votes from $P_1$ creating \ccc{$V_1$}. $D^\prime$ proposes $V_2$ to $P_2$ and gathers votes but cannot form a \cc.

\item Create the following partitions: $P_1=\{D,E\}$, $P_2=\{\underline{D^\prime},F\}$, $P_3=\{\underline{G}\}$.

\item $D$ broadcasts \ccc{$V_1$}, which only reaches $P_1$ \ie $(D,E)$.

\end{itemize}

% -------- Step 3 ------

\item [Step 3] Drop all proposals from $D$ and $D^\prime$ until a new view starts. \alberto{I prefer the terminology "drop all proposals" rather than "delay all messages until a new view"; even better "drop all proposals by isolating each nodes into mutually disjoints partitions"} View 2:

\begin{itemize}

\item Remove all partitions, \ie: $P=\{D,D^\prime,E,\underline{F},G\}$.

\item Let $F$ run as leader for one round. $F$ re-proposes $V_2$ (\ie $D^\prime$'s proposal in the previous round) to $P$. $(D,E)$ do not vote because they already have \ccc{$V_1$} for that height. $F$ gathers votes from rest of the nodes and forms \ccc{$V_2$}.

\item Create the following partitions: $P_1=\{D,E\}$, $P_2=\{\underline{D^\prime},F\}$, $P_3=\{\underline{G}\}$.

\item $F$ broadcasts \ccc{$V_2$}, which only reaches $P_2$ \ie $(D^\prime,F)$.

\end{itemize}

% -------- Step 4 ------

\item [Step 4] Drop all proposals from $F$ until new view starts. View 3:

\begin{itemize}

\item Create the following partitions: $P_1=\{D,\underline{E},G\}$, $P_2=\{\underline{D^\prime},F\}$.

\item Let $E$ run as leader for one round. $E$ proposes $V_3$ which extends the highest \cc it knows \ccc{$V_1$}. As before, $E$ manages to form \ccc{$V_3$}, but as a result of a partition, the \cc will only reach $(D,E)$. Next, there is a view-change, $F$ is the new leader, and there are no partitions. $F$ proposes $V_4$ which extends \ccc{$V_2$}, the highest \cc it knows. However, $(D ,E)$ do not vote because $V_4$ does not extend their highest \cc \ie \ccc{$V_3$}. This scenario can repeat indefinitely, resulting in the loss of liveness.   

\end{itemize}

\end{description}

